Impulse Stability of Large Flocks: an Example

Consider a string of N+1 damped oscillators moving on the line of which the motion of the first (called the "leader") is independent of the others. Each of the followers `observes' the relative velocity and position of only its nearest neighbors. Inasmuch as these are different from 0, this information is then used to determine its own acceleration. Fix all parameters except the number N in such a way that the system is asymptotically stable. Now as N tends tends we consider the following problem. At t=0 the leader gets kicked and starts moving with unit velocity away from the flock. Due to asymptotic stability the followers will eventually fall in behind the leader and travel each at its own predetermined distance from the leader. In this note we conjecture that before equilibrium ensues, the perturbations to the orbit of the last oscillator grow exponentially in N except when there is a symmetry in the interactions and the growth is then linear in N. There are two cases. We prove the conjecture in one case, and give a strong heuristic argument in the other.

==> inputlatex.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%To draw commutative diagrams.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amscd}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}

\textwidth=18.00 true cm \textheight=21.50 true cm
\baselineskip=18pt \voffset=-2cm \hoffset=-2.5cm
%\parskip=8pt
\parindent=6ex
%\input{pepet.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%Valencian Definitions
%Uso de las definiciones valencianas%
%Theorem
%\begin{theo}\label{***}Statement of theorem \end{theo}
%\begin{prop}\label{***}Statement of theorem \end{prop}
%\begin{lem}\label{***}Statement of theorem \end{lem}
%\begin{cory}\label{***}Statement of theorem \end{cory}
%\begin{rem}\label{***}Statement of theorem \end{rem}
%when needed:
%\setcounter{figure}{0}
%\setcounter{equation}{0}
%\setcounter{theorem}{0}
%\begin{proof}  Proof \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\renewcommand{\thefigure}{\thesection.\arabic{figure}}
\newtheorem {theo} {\bf Theorem} [section]
\newtheorem {prop} [theo] {\bf Proposition}
\newtheorem {cory} [theo] {\bf Corollary}
\newtheorem {lem} [theo] {\bf Lemma}
\newtheorem {defn} [theo] {\bf Definition}
\newtheorem {conj} [theo] {\bf Conjecture}
\newtheorem {exam} [theo] {\bf Example}
\newtheorem {rem} [theo] {\bf Remark}
\newcommand{\QED}{\hfill \CaixaPreta \vspace{6mm}}
\def\CaixaPreta{\vrule Depth0pt height6pt width6pt}
\newenvironment{remark}{\begin{rem}\begin{rm}}{\end{rm}
\nopagebreak\hfill$\Box$\end{rem}\par\vspace{\partopsep}}
\newenvironment{defin}{\begin{DEFCURSIVA}\begin{rm}}{\end{rm}\end{DEFCURSIVA}}
\newenvironment{proclama}[1]{\par\vspace{\topsep}\noindent{\bf #1}
\begin{em}}{\end{em}\par\vspace{\topsep}}
\newcommand{\qed}{\nopagebreak\hfill{\vrule width6pt height6pt depth0pt}}
%\newenvironment{proof}{\noindent{\bf Proof:}}{\qed\par
%\vspace{\topsep}\vspace{\partopsep}}
\newenvironment{proof}[1]{\vspace{0.4 cm}\noindent{\em #1.}}{\qed\par
\vspace{\topsep}\vspace{\partopsep}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dpy}{\displaystyle}
%eqn array with numbered lines:
%use & to align, \\ for new line, \\[0.4cm] for new line and add'l vert. space.
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
%eqn array no number:
\newcommand{\benn}{\begin{eqnarray*}}
\newcommand{\eenn}{\end{eqnarray*}}
%single eqn numbered:
\newcommand{\bse}{\begin{equation}}
\newcommand{\ese}{\end{equation}}
%single eqn no number:
\newcommand{\bsenn}{\begin{displaymath}}
\newcommand{\esenn}{\end{displaymath}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Some Functions (math style)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\logand}{\;\;{\rm and }\;\;}
\newcommand{\for}{\;\;{\rm for }\;\;}
\newcommand{\logor}{\;\;{\rm or }\;\;}
\newcommand{\logif}{\;\;{\rm if }\;\;}
\newcommand{\logelse}{\;\;{\rm else }\;\;}
\newcommand{\then}{\;\;{\rm then }\;\;}
\newcommand{\where}{\;\;{\rm where }\;\;}
\newcommand{\with}{\;\;{\rm with }\;\;}
\newcommand{\such}{\;\;{\rm such\; that }\;\;}
\newcommand{\limcap}{\;{\rm d }\,}
\newcommand{\Tr}{\;{\rm Tr }\,}
\newcommand{\Hd}{\;{\rm Hd }\,}
\newcommand{\atanh}{\;{\rm arctanh }\,}
\newcommand{\Hdim}{\;{\rm Hdim }\,}
\newcommand{\Hlim}{\;{\rm Hlim }\,}
\newcommand{\card}{\;{\rm card }\,}
\newcommand{\Id}{\,{\rm Id}\,}
%\newcommand{\mod}{\bmod}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Other
%%('re' is added because \O and \S are existing commands)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\C}{\mbox{I${\!\!\!}$C}}
\renewcommand{\O}{\mbox{I${\!\!\!}$O}}
\renewcommand{\H}{\mbox{I${\!\!\!}$H}}
\newcommand{\Q}{\mbox{I${\!\!\!}$Q}}
\newcommand{\G}{\mbox{I${\!\!\!}$G}}
\newcommand{\T}{\mbox{T${\!\!\!}$T}}
\newcommand{\N}{\mbox{I${\!}$N}}
\newcommand{\R}{\mbox{I${\!}$R}}
\newcommand{\D}{\mbox{I${\!}$D}}
\newcommand{\Z}{\mbox{Z${\!\!}$Z}}
\renewcommand{\S}{\mbox{S${\!\!\!\!}$S}}
\newcommand{\CaixaBranca}{$\Box$}
\newcommand{\creu}{{\rule[-0.1mm]{2mm}{0.2mm}\rule{0.1mm}{2.5mm}}}
\newcommand{\ca}{\c ca }
\newcommand{\co}{\c co }
\newcommand{\mv}{mente, }
\newcommand{\caop}{\c c\~ao. }
\newcommand{\caov}{\c c\~ao, }
\newcommand{\coesp}{\c c\~oes. }
\newcommand{\coesv}{\c c\~oes, }
\newcommand{\cao}{\c c\~ao }
\newcommand{\CAO}{\c C\~AO }
\newcommand{\coes}{\c c\~oes }
\newcommand{\COES}{\c C\~OES }
\newcommand{\sao}{s\~ao }
\newcommand{\SAO}{S\~AO }
\newcommand{\m}{mente }
\newcommand{\ii}{\'{\i}}

